Learning Harmonized Representations for Speculative Sampling

Speculative sampling is a promising approach to accelerate the decoding stage for Large Language Models (LLMs). Recent advancements that leverage target LLM's contextual information, such as hidden states and KV cache, have shown significant practical improvements. However, these approaches suffer from inconsistent context between training and decoding. We also observe another discrepancy between the training and decoding objectives in existing speculative sampling methods. In this work, we propose a solution named HArmonized Speculative Sampling (HASS) that learns harmonized representations to address these issues. HASS accelerates the decoding stage without adding inference overhead through harmonized objective distillation and harmonized context alignment. Experiments on four LLaMA models demonstrate that HASS achieves 2.81x-4.05x wall-clock time speedup ratio averaging across three datasets, surpassing EAGLE-2 by 8%-20%. The code is available at https://github.com/HArmonizedSS/HASS.

==> algorithm/context_alignment.tex <==
\begin{algorithm}
\setstretch{1.1}
\caption{Harmonized Context Alignment}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Number of training steps $J$, token embedding $e = \{e_{i}\}_{i=0}^{t+1}$, target LLM $\mathcal{M}^{(l)}(e_{in}, m_{in})$, draft model $\mathcal{M}^{(s)}(e_{in}, q_{in}, kv_{in}, m_{in})$, language model head $\mathcal{H}(f_{in})$, feature loss function $\mathcal{L}_{fea}(f_t, f_p)$, logit loss function $\mathcal{L}_{logit}(l_t, l_p)$.\textcolor[rgb]{0.31,0.65,0.38}{\COMMENT{Input embedding $e_{in}$, query feature $q_{in}$, key\&value feature $kv_{in}$, attention mask $m_{in}$, input feature $f_{in}$, target feature $f_{t}$, predicted feature $f_{p}$, target logit $l_{t}$, predicted logit $l_{p}$}}
\STATE Get causal attention mask $m_{causal}$ as that in `HASS Training Step 1' of Figure \ref{fig:multi-step alignment};
\STATE $f^{(l)} \leftarrow f^{(l)}_{:t+1} = \mathcal{M}^{(l)}(e_{in}=e_{:t+1}, m_{in}=m_{causal})$;\textcolor[rgb]{0.31,0.65,0.38}{\COMMENT{Generate target LLM feature}}
\STATE $f^{(s_{1})} \leftarrow f^{(s_{1})}_{1:t+2} = \mathcal{M}^{(s)}(e_{in}=e_{1:t+2}, qkv_{in}=f^{(l)}, m_{in}=m_{causal})$;\textcolor[rgb]{0.31,0.65,0.38}{\COMMENT{First draft forward}}
\STATE $l^{(l)}, l^{(s_1)} \leftarrow \mathcal{H}(f^{(l)}), \mathcal{H}(f^{(s_1)})$;\textcolor[rgb]{0.31,0.65,0.38}{\COMMENT{Compute logits for target LLM and draft model}}
\STATE $L_{1} = \mathcal{L}_{fea}(f^{(l)}_{1:t+1}, f^{(s_1)}_{1:t+1}) + \mathcal{L}_{logit}(l^{(l)}_{1:t+1}, l^{(s_1)}_{1:t+1})$;\textcolor[rgb]{0.31,0.65,0.38}{\COMMENT{Combine feature loss and logit loss}}
\STATE Update $\mathcal{M}^{(s)}$ with the loss $L_{1}$;
\STATE \textbf{for} $j=2$ \textbf{to} $J$ \textbf{do}
\STATE \qquad Get modified attention mask $m_{j}$ as that in `HASS Training Step $j$' of Figure \ref{fig:multi-step alignment};
\STATE \qquad Set $\hat{f}^{(s_{j-1})} \leftarrow f^{(l)}_{0} \oplus f^{(s_{1})}_{1} \oplus \cdots \oplus f^{(s_{j-1})}_{j:t+1}$;\textcolor[rgb]{0.31,0.65,0.38}{\COMMENT{Prepare query feature}}
\STATE \qquad Set $F_j \leftarrow [f^{(l)},\hat{f}^{(s_{1})},\cdots,\hat{f}^{(s_{j-1})}]$;\textcolor[rgb]{0.31,0.65,0.38}{\COMMENT{Prepare key\&value feature}}
\STATE \qquad $f^{(s_{j})} \leftarrow \mathcal{M}^{(s)}(e_{in}=e_{1:t+2}, q_{in}=\hat{f}^{(s_{j-1})}, kv_{in}=F_j, m_{in}=m_{j})$;\textcolor[rgb]{0.31,0.65,0.38}{\COMMENT{$j$-th draft forward}}
\STATE \qquad $l^{(s_j)} \leftarrow \mathcal{H}(f^{(s_j)})$;
\STATE \qquad $L_{j} = \mathcal{L}_{fea}(f^{(l)}_{1:t+1}, f^{(s_j)}_{1:t+1}) + \mathcal{L}_{logit}(l^{(l)}_{1:t+1}, l^{(s_j)}_{1:t+1})$;
\STATE \qquad Update $\mathcal{M}^{(s)}$ with the loss $L_{j}$;
\STATE \textbf{end for}
\STATE \textbf{Output:} Updated draft model $\mathcal{M}^{(s)}$.
\end{algorithmic}
\end{algorithm}

==> table/ablation_align.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht]
\centering
\resizebox{320pt}{!}{
\begin{tabular}{cccccccccc}
\toprule
                     &      & \multicolumn{2}{c}{MT-bench} & \multicolumn{2}{c}{HumanEval} & \multicolumn{2}{c}{GSM8K} & \multicolumn{2}{c}{Mean} \\ \midrule
                     & Aligning Step & Speedup          &$\tau$        & Speedup          &$\tau$         & Speedup        &$\tau$       & Speedup         &$\tau$       \\ \midrule
\multirow{5}{*}{T=0} & EAGLE-2 + Top-K    &         2.68x         &     4.59      &        3.13x          &     4.97       &         3.08x       &     4.77     &         2.96x        &    4.78      \\
                     & HASS Align-2    &         2.93x         &      4.95     &        3.39x          &      5.25      &         3.09x       &      5.12    &    3.14x            &     5.11    \\
                     & HASS Align-3    &          2.99x        &     \textbf{4.99}      &  3.41x                &     5.29       &     \textbf{3.32x}           &     5.17    &       \textbf{3.24x}         &     5.15     \\
                     & HASS Align-4    &         \textbf{3.04x}         &    \textbf{4.99}       &         \textbf{3.44x}         &     \textbf{5.30}       &        \textbf{3.24x}       &    \textbf{5.18}     &   3.24x            &     \textbf{5.16}    \\
                     & HASS Align-5    &        2.82x          &     4.98      &          3.26x        &       5.26     &     3.08x        &    5.09    &       3.05x         &     5.11    \\ \midrule
\multirow{5}{*}{T=1} & EAGLE-2 + Top-K    &          2.41x        &      4.46     &         2.89x         &      4.61      &        2.42x       &    4.64    &         2.57x       &    4.57    \\
                     & HASS Align-2    &        2.63x          &    4.71       &         3.03x         &       4.89     &       2.82x        &    4.98     &      2.83x           &    4.86      \\
                     & HASS Align-3    &          2.70x        &     \textbf{4.84}      &          3.13x        &      4.91      &    \textbf{2.87x}           &    5.01    &        2.90x        &     \textbf{4.92}     \\
                     & HASS Align-4    &          \textbf{2.76x}        &    4.77       &         \textbf{3.14x}         &     \textbf{4.93}       &    2.86x        &     \textbf{5.03}    &        \textbf{2.92x}       &    4.91    \\
                     & HASS Align-5    &         2.59x         &      4.71     &         2.96x        &     4.92       &         2.82x       &     4.95    &    2.79x            &    4.86    \\ \bottomrule
\end{tabular}
}
\caption{Speedup ratios and acceptance length of HASS with varied aligning step in the context-aware alignment. GSM8K-ZS}
\label{ablation: align}
\end{table}

==> table/ablation_hyper_tau.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht]
\centering
\Huge
\resizebox{395pt}{!}{
\begin{tabular}{cc|cccc|cccc|cccc|cccc|cccc}
\toprule
\multicolumn{2}{c}{Depth}     & \multicolumn{4}{c}{5} & \multicolumn{4}{c}{6} & \multicolumn{4}{c}{7} & \multicolumn{4}{c}{8} & \multicolumn{4}{c}{9} \\
\multicolumn{2}{c}{Tokens}    & 40  & 60  & 80  & \multicolumn{1}{c}{100} & 40  & 60  & 80  & \multicolumn{1}{c}{100} & 40  & 60  & 80  & \multicolumn{1}{c}{100} & 40  & 60  & 80  & \multicolumn{1}{c}{100} & 40  & 60  & 80  & 100 \\ \midrule
\multirow{3}{*}{T=0} & L2 7B  &  4.73   &  4.85   &  4.94   &  4.98   &  5.07   &  5.25   &  5.36   &   5.41  &  5.32   &  5.53   &  5.64   &  5.76   &  5.46   &  5.70   &   5.86  &  6.00   &  5.63   &  5.87   &  6.04   &   6.18  \\
                     & L2 13B &  4.74   &  4.87   &  4.93   &  4.97   &   5.07  &  5.27   &  5.37   &  5.43   &  5.28   &   5.52  &   5.65  &  5.73   &   5.45  &  5.68   &  5.85   &  5.96   &   5.57  &  5.82   &  6.03   &  6.15   \\
                     & L3 8B  &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     \\ \midrule
\multirow{3}{*}{T=1} & L2 7B  &  4.51   &  4.68   &   4.72  &  4.79   &  4.71   &  4.97   &   5.08  &  5.10   &  4.94   &  5.17   &  5.27   &   5.32  &  5.07   &  5.21   &  5.45   &   5.57  &  5.10   &  5.37   &  5.60   &   5.66  \\
                     & L2 13B &  4.55   &  4.72   &  4.76   &  4.78   &   4.88  &  5.02   &  5.14   &  5.25   &  5.09   &   5.26  &   5.41  &  5.49   &  5.18   &  5.38   &  5.48   &  5.67   & 5.20    &   5.55  &   5.76  &   5.89  \\
                     & L3 8B  &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     \\ \bottomrule
\end{tabular}
}
\caption{Acceptance length of HASS-MG with varied depths and total tokens.}
\label{ablation: hyper-tau}
\end{table}

==> table/ablation_reweight.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht]
\tiny
\centering
\resizebox{190pt}{!}{
\begin{tabular}{cccc}
\toprule
Reweight Factor & T = 0  & T = 1  & Mean \\ \midrule
1.0 (Default)    & 4.62 & 4.59 & 4.61 \\
0.7    & 4.65 & 4.61 & 4.63 \\
0.5    & \textbf{4.67} & \textbf{4.62} & \textbf{4.65} \\ \bottomrule
\end{tabular}
}
\caption{Acceptance lengths $\tau$ of HASS with different reweight factors for harmonized context alignment. The results are conducted on LLaMA3-Instruct 70B over MT-bench dataset with temperature T $\in \{0, 1\}$.}
\label{ablation: reweight}
\end{table}
